Can transformative AI shape a new age for our civilization?: Navigating between speculation and reality

Artificial Intelligence is widely regarded as a transformative force with the potential to redefine numerous sectors of human civilization. While Artificial Intelligence has evolved from speculative fiction to a pivotal element of technological progress, its role as a truly transformative agent, or transformative Artificial Intelligence, remains a subject of debate. This work explores the historical precedents of technological breakthroughs, examining whether Artificial Intelligence can achieve a comparable impact, and it delves into various ethical frameworks that shape the perception and development of Artificial Intelligence. Additionally, it considers the societal, technical, and regulatory challenges that must be addressed for Artificial Intelligence to become a catalyst for global change. We also examine not only the strategies and methodologies that could lead to transformative Artificial Intelligence but also the barriers that could ultimately make these goals unattainable. We end with a critical inquiry into whether reaching a transformative Artificial Intelligence might compel humanity to adopt an entirely new ethical approach, tailored to the complexities of advanced Artificial Intelligence. By addressing the ethical, social, and scientific dimensions of Artificial Intelligence's development, this work contributes to the broader discourse on the long-term implications of Artificial Intelligence and its capacity to drive civilization toward a new era of progress or, conversely, exacerbate existing inequalities and risks.

==> chapters/part_2.tex <==
\chapter[The Computational Intelligence behind TAI]{PART II: The Computational Intelligence behind Transformative AI}\label{theors_approach}

\input{chapters/theor_foundations}

==> chapters/theor_foundations.tex <==
\section{BCAI Is Not the Only Way to TAI}\label{tai_without_bcai}

\begin{quote}
    ``\textit{The question of whether machines can think is about as relevant as the question of whether submarines can swim.}''
    \\
    --- \textit{Edsger W. Dijkstra}
\end{quote} 

The Dijkstra's quote underscores the notion that comparing the ability of machines to think with human's cognitive processes is as misplaced as comparing the ability of submarines to swim with that of a fish. He then challenged the relevance of the question by highlighting a fundamental misalignment in analogies. We would like to reinterpret this quote to critique the way that many individuals approach the concept of AI. 

Dijkstra argued that asking whether machines can ``think'' is a fundamentally misguided question, as it applies a biological concept (human thought) to machines, in much the same way that it would be inappropriate to ask whether submarines ``swim'', a term that describes a biological function. Submarines move underwater, but in a manner entirely distinct from how living organisms swim. By analogy, machines can perform tasks that resemble human thought processes, yet they do so using methods that differ fundamentally from human cognition. Dijkstra’s point emphasizes that the discourse on AI should not be concerned with whether AI can think in the human sense, but rather with whether they can autonomously and effectively perform complex tasks. His statement highlights the importance of recognizing that the value and utility of machines do not depend on their capability to replicate human thinking and skills identically, but on their ability to achieve similar outcomes through different means. In light of recent AI advances, we have seen that it is not essential to possess an AI with exceptionally sophisticated capabilities to continue driving progress. In this sense, while the human brain has undeniably inspired much of the development of contemporary AI (e.g. neural networks) \citep{ren2024brain,wang2024brain}, it does not necessarily need to serve as the definitive blueprint for its design. The brain can provide a reference for what intelligence achieves (e.g. reasoning, learning, and decision-making), but not necessarily how these capabilities must be implemented. This distinction echoes Dijkstra's quote where this reinterpretation is intended to show how AI systems can diverge from biological intelligence in structure and function, while achieving equally transformative results. By freeing AI development from strict adherence to neural emulation, researchers could explore novel architectures and approaches that optimize for different goals, constraints, and capabilities, potentially surpassing the limitations of human cognition in certain contexts. This conceptual flexibility underscores the potential of AI as an innovation not constrained by biology, but rather informed by it \citep{zhao2022inspired,gershman2024have}.

Therefore, AI could transition to \texttt{TAI} without the necessity of progressing through \texttt{BCAI} (as illustrated by Dijkstra's quote). However, it is indeed the case that the latter pathway is the one most commonly associated with the concept of \texttt{TAI}. Consequently, this part will examine some of the most widely discussed theoretical arguments both in favor of and against this possibility.

The development of \texttt{BCAI} may be underpinned by a complex interplay of theoretical foundations and inherent limitations derived from fundamental theorems in Computer Science, Mathematics, and Information Theory. These frameworks provide essential insights into the capabilities and constraints of computational systems, shaping the possibilities of achieving \texttt{BCAI}. Therefore, this part explores their dual nature, examining how they support or challenge the realization of \texttt{BCAI}. By analyzing their implications, this discussion aims to provide a balanced perspective on the theoretical landscape of \texttt{TAI}, emphasizing areas where innovation and practical trade-offs are essential for progress. The synthesis of these diverse perspectives (see Table \ref{tab:theorems_bcai}) reveals not only the immense potential of \texttt{TAI} but also the profound challenges it faces as an inherently computational endeavor.

\begin{table}[H]
\centering
\renewcommand{\arraystretch}{1.5}
\resizebox{0.7\textwidth}{!}{ % Scale to 80% of text width
\begin{tabularx}{\textwidth}{@{}>{\centering\arraybackslash}p{3cm}X>{\centering\arraybackslash}p{3cm}@{}}
\toprule
\textbf{Theorem} & \textbf{Key Contribution and Limitation for \texttt{BCAI}} & \textbf{Role} \\ 
\midrule
\texttt{Turing Completeness} & Demonstrates that any computable process can be simulated by a Turing machine, enabling universal computation. However, it cannot solve non-computable problems, such as the Halting Problem, which imposes inherent limits on predictability. & Foundational enabler of computation and \texttt{BCAI} feasibility. \\ 
\texttt{Universal Approximation Theorem} & Establishes that neural networks can approximate any continuous function, supporting \texttt{BCAI} in modeling complex cognitive tasks. Practical issues like overfitting and training inefficiencies, however, limit scalability. & Supports flexibility and adaptability in learning systems. \\ 
\texttt{Bayesian Inference} & Provides a framework for reasoning under uncertainty, essential for \texttt{BCAI} adaptability. Yet, the computational cost in high-dimensional spaces can hinder its real-world application. & Enables probabilistic reasoning and robust decision-making. \\ 
\texttt{Hutter's Universal AI} & Defines a theoretically optimal agent for decision-making in computable environments. However, its reliance on computationally intractable methods, like Solomonoff induction, makes implementation infeasible. & Provides an idealized framework for \texttt{BCAI} optimization. \\ 
\texttt{Algorithmic Information Theory} & Offers principles for efficient data representation and generalization, essential for learning. Nonetheless, undecidability in finding minimal representations constrains \texttt{BCAI}'s optimization. & Enables efficient encoding and generalization but highlights inherent limitations. \\ 
\texttt{G\"odel's Incompleteness Theorem} & Highlights that some truths in formal systems are undecidable, limiting \texttt{BCAI}'s ability to achieve complete reasoning. Encourages modular and approximate reasoning approaches. & Limits comprehensive reasoning and universal consistency. \\ 
\texttt{Halting Problem} & Demonstrates that no algorithm can universally predict program termination, impacting \texttt{BCAI}'s reliability in dynamic systems. Promotes modular and bounded problem-solving to mitigate this limitation. & Highlights unpredictability and promotes bounded approaches. \\ 
\texttt{Complexity Theory} & Suggests that many real-world problems are computationally intractable if $P \neq NP$, posing scalability challenges for \texttt{BCAI}. Approximation methods provide a workaround for bounded domains. & Exposes scalability challenges and promotes heuristic solutions. \\ 
\texttt{Shannon’s Information Theory} & Enables efficient data compression and communication, vital for large-scale AI systems. However, limits on channel capacity and noise robustness can constrain reliability. & Supports efficient data handling but imposes communication limits. \\ 
\texttt{Rice's Theorem} & States that non-trivial properties of program behavior are undecidable, preventing \texttt{BCAI} from fully analyzing or verifying the behavior of itself or other systems. Encourages heuristic and probabilistic approaches. & Constrains self-analysis and system verification. \\ 
\bottomrule
\end{tabularx}
}
\caption{Comparative overview of the most accepted Computational Intelligence theorems, with their roles and their impact on achieving \texttt{BCAI}.}
\label{tab:theorems_bcai}
\end{table}

\section{Theorems Supporting and Challenging BCAI}\label{theors_yes_no}

\subsection{Turing Completeness}\label{turing_comp}
Turing completeness \citep{turing1936computable} establishes the theoretical foundation for universal computation. A Turing-complete system can simulate any computation given sufficient time and resources. This universality implies that any algorithmic cognitive process, including those underlying human intelligence, can, in principle, be implemented on a computational system. Turing completeness thus supports \texttt{BCAI} by asserting that all computable aspects of human reasoning, learning, and problem-solving can be reproduced. However, it is worth noting that this theory applies only to computable functions, leaving undecidable problems beyond its scope. Nonetheless, Turing completeness underpins the theoretical possibility of \texttt{BCAI}, as human cognition, if reducible to algorithmic models, can be executed on Turing machines or equivalent systems \citep{turing2009computing}. While Turing completeness guarantees the theoretical feasibility of implementing any computable process, several practical challenges remain for achieving \texttt{BCAI}, such as the efficiency of computation (e.g. time and memory) or that only applies to computable functions.

\subsection{Universal Approximation Theorem}\label{universal_app}
This theorem first formalized in \citep{cybenko1989approximation} and later generalized in \citep{hornik1991approximation}, states that a neural network with a sufficient number of neurons in a single hidden layer can approximate any continuous function on a compact subset of $\mathbb{R}^n$, i.e. the n-dimensional Euclidean space. This result demonstrates the theoretical capacity of neural networks to model complex relationships and dynamics inherent in cognitive processes. It supports \texttt{BCAI} by providing the mathematical foundation for deep learning models to approximate and potentially surpass human-level capabilities in various domains. However, practical challenges, such as overfitting, training inefficiencies, and data availability, limit its immediate applicability to \texttt{BCAI}. Nonetheless, it highlights the potential of neural networks to approximate complex functions, which does not directly address the ability to generalize cognitive functions akin to human intelligence.

\subsection{Bayesian Inference}\label{bayes_inf}
Bayesian inference, rooted in Bayes’ Theorem \citep{bayes1763essay}, offers a framework for reasoning under uncertainty by updating probabilities as new evidence becomes available. This methodology is critical for \texttt{BCAI}, as it enables systems to adapt dynamically to incomplete or noisy data, an essential feature for real-world applications. Bayesian inference supports \texttt{BCAI} by formalizing how can process uncertain environments more systematically and effectively than humans, who are prone to cognitive biases. However, it also introduces limitations, as priors must be carefully defined, and the computational cost of Bayesian methods can be prohibitive in high-dimensional scenarios. Despite these challenges, Bayesian reasoning is fundamental for creating adaptive and robust \texttt{BCAI} \citep{pearl2009causality,gerstenberg2024counterfactual}. 

\subsection{Algorithmic Information Theory}\label{ait_th}
The Algorithmic information theory \citep{solomonoff1964formal,kolmogorov1965three} defines the complexity of data as the length of the shortest program that can generate it. This principle supports \texttt{BCAI} by formalizing how intelligent systems can identify and generalize patterns efficiently. It aligns with Occam’s Razor \citep{blumer1987occams}, prioritizing simpler models that generalize better. However, the theory imposes a fundamental limitation: computing the minimal program is undecidable. This constraint means that while \texttt{BCAI} could approach optimal generalization, it cannot achieve perfect model minimality. Nonetheless, algorithmic information theory provides a foundational framework for building systems that learn efficiently.

\subsection{Hutter's Universal AI}\label{hutter_th}
The Marcus Hutter’s Universal AI framework \citep{hutter2005universal} introduces the AIXI model as a theoretical \texttt{BCAI} agent. AIXI combines Solomonoff induction \citep{solomonoff1964formal} with reinforcement learning to achieve optimal decision-making in any computable environment. By leveraging simplicity and Bayesian principles, AIXI represents a theoretically \texttt{BCAI} capable of surpassing human intelligence in well-defined tasks. However, its reliance on Solomonoff induction makes AIXI computationally intractable, as it involves summing over all possible hypotheses weighted by complexity. Despite this, Hutter's work provides a formal definition of \texttt{BCAI}, reinforcing the theoretical possibility of \texttt{BCAI} while highlighting significant practical barriers.

\subsection{The G\"odel's Incompleteness Theorem}\label{godel_th}
It demonstrates that in any consistent formal system capable of expressing basic arithmetic, there are true statements that cannot be proven within the system \citep{godel1931formal}. This theorem imposes a fundamental limitation on \texttt{BCAI} by highlighting the inherent incompleteness of formal reasoning frameworks. While it does not negate the possibility of \texttt{BCAI}, it suggests that such systems may encounter problems analogous to G\"odel's sentences (true but undecidable). This limitation implies that \texttt{BCAI} could not fully replicate or surpass human reasoning in every domain, as it may fail to address inherently undecidable questions. This theorem challenges the idea that the universe, human cognition, or mathematics can be completely understood through mechanistic or algorithmic means.

\subsection{Chaitin's Incompleteness Theorem}\label{chaitin_th}
It extends G\"odel's work to algorithmic information theory, demonstrating that there are limits to what can be proven about the complexity of programs within formal systems \citep{chaitin1974information}. This imposes a constraint on \texttt{BCAI} by highlighting the impossibility of finding the shortest or most efficient representations for all problems. While \texttt{BCAI} could approximate solutions, it cannot guarantee optimality in all cases. Chaitin's Theorem underscores the trade-offs between precision, computational cost, and practical feasibility in \texttt{BCAI} development. 

\subsection{Rice's Theorem}\label{rice_th}
The Rice's Theorem \citep{rice1953classes} poses a fundamental challenge to the realization of \texttt{BCAI} by establishing that any non-trivial property of a program’s behavior is undecidable. This result implies that a \texttt{BCAI} system cannot universally and algorithmically determine whether another program (or even itself) exhibits certain desirable properties, such as safety, ethical alignment, or performance optimization. For instance, a \texttt{BCAI} attempting to analyze or verify its own modifications during a process of recursive self-improvement would encounter inherent computational barriers, as verifying whether such modifications improve functionality or maintain alignment with human values is undecidable for non-trivial cases. This limitation extends to the prediction of the behavior of external agents or systems, particularly in complex, dynamic environments, where \texttt{BCAI} systems are expected to generalize and adapt. Consequently, Rice's Theorem highlights the need for \texttt{BCAI} to rely on heuristic methods, probabilistic reasoning, or domain-specific constraints to mitigate these challenges, underscoring the complexity of ensuring safe and reliable intelligence in general-purpose systems.

\subsection{The Halting Problem}\label{halting_problem}
The Halting Problem \citep{lucas2021origins} is a decision problem in computability theory, proving that there is no general algorithm capable of deciding whether any arbitrary program halts or runs indefinitely, and it relates closely to other fundamental results (the G\"odel’s incompleteness Theorem \citep{godel1931formal} Theorem, the Chaitin's incompleteness \citep{chaitin1974information} Theorem, and the Rice's Theorem \citep{rice1953classes}). This limitation affects \texttt{BCAI} tasked with verifying program behavior or predicting the termination of dynamic processes. It imposes a theoretical barrier to perfect prediction in self-referential or open-ended systems. The Halting Problem directly impacts the design and limits of \texttt{BCAI}, particularly in areas of reasoning, predictability, and self-analysis.

\subsection{Complexity Theory}\label{complex_th}
The unresolved $P$ vs $NP$ problem \citep{cook1971complexity} questions whether every problem whose solution can be verified in polynomial time $NP$ can also be solved in polynomial time $P$. If $P \neq NP$, many critical problems, including optimization and decision-making tasks relevant to \texttt{BCAI}, are computationally intractable. While heuristic and approximate methods can address specific cases, \texttt{BCAI} would face fundamental limits in solving $NP$-complete problems optimally. Complexity theory thus imposes scalability constraints, suggesting that \texttt{BCAI} systems may excel in bounded domains, but struggle with large-scale real-world complexities.

\subsection{Shannon's Information Theory}\label{shannon_th}
The Shannon’s Information Theory \citep{shannon1948mathematical} provides essential tools for optimizing data compression, transmission, and error correction, enabling \texttt{BCAI} to handle vast datasets efficiently. However, the Channel Capacity Theorem imposes hard limits on reliable data transmission, particularly in noisy environments. These constraints can hinder \texttt{BCAI} systems reliant on real-time communication or distributed architectures. Additionally, Shannon’s entropy does not distinguish between meaningful signals and noise, leaving \texttt{BCAI} vulnerable to misinformation or adversarial attacks. While supportive in data handling, Information Theory highlights practical barriers to scaling \texttt{BCAI} robustly.

\vspace{\baselineskip}

Let us dwell more on the point that deals with entropy, as it is of special importance in the achievement of \texttt{BCAI}. Shannon's Information Theory relates to cross-entropy \citep{thomas2006elements}, and this is especially relevant because is the basis of many machine learning approaches and variants (e.g. decision trees, neural networks, reinforcement learning, autoencoders, even the famous LLMs). Cross-entropy is used as the loss function during training, which goal is to minimize this loss, which at the same time means reducing the discrepancy between the model predictions and the true distribution. However, there are limits to what cross-entropy minimization can achieve when trying to achieve \texttt{BCAI} behavior. Reducing cross-entropy improves efficiency in information handling, but does not imply that the model has a deep understanding of the concepts it manipulates. A \texttt{BCAI} would require knowledge beyond statistical correlation, implying an ability to model the world and reason about it (e.g. causality \citep{pearl2009causality}), which is not achieved by mere entropy optimization. Moreover, in Information Theory, minimizing entropy is synonymous with finding an efficient encoding of information. For a \texttt{BCAI}, the issue is not only to encode efficiently, but to integrate and use that information to make decisions in varied and unknown environments. This is something that cannot be achieved solely by tuning a model to accurately predict a data set. Finally, entropy and Kolmogorov complexity are related to each other, as the latter measures the minimum length of an object's description. If e.g. an LLM is trained to minimize a cross-entropy loss, it is in a way approximating a more efficient description of its data set. \texttt{BCAI}, however, should be able to understand the underlying ``structure'' of reality, not just find a compact way to describe its observations. 

In summary, Shannon's Information Theory and cross-entropy are crucial for understanding how machine learning works and for evaluating their predictive performance. However, these concepts, while powerful, also highlight the limitations of these models when compared to the requirements for achieving \texttt{BCAI}. Cross-entropy allows measuring how well a model fits the data, but it is not sufficient to capture the depth and breadth of human intelligence, which involves skills such as abstract reasoning, adapting to unprecedented situations, and building a coherent model of the world. Consequently, we may need something beyond this theory to achieve \texttt{BCAI}.

\vspace{\baselineskip}

So far our discussions have exposed that the same theorem may support or reject at the same time the possibility to reach \texttt{BCAI}. We have even seen that one theorem can be a limiting factor for another theoretical framework. The chains in Figure \ref{fig:BCAI_supp} represent conceptual or logical relationships between computational theorems, highlighting how their principles interact to either support or limit the feasibility of achieving \texttt{BCAI}. These chains show the flow of ideas and dependencies among the theorems. For example, the main supportive chain (Turing Completeness $\mapsto$ Universal Approximation Theorem $\mapsto$ Bayesian Inference) provides a pathway for \texttt{BCAI} to simulate, learn, and reason across complex tasks. In contrast, the main limiting chain (Halting Problem $\mapsto$ G\"odel's Incompleteness Theorem $\mapsto$ Rice's Theorem) highlights cascading barriers to predictability, reasoning, and self-analysis. Meanwhile, cross-domain insights from Shannon’s Information Theory and Algorithmic Information Theory reveal both the potential for efficient computation and the inherent trade-offs of these approaches. In these ambivalent chains (Shannon’s Information Theory $\mapsto$ Algorithmic Information Theory), we observe that 1) Shannon’s Information Theory enables efficient data compression and error correction, crucial for managing the large datasets needed by \texttt{BCAI}; and 2) that Algorithmic Information Theory extends this by emphasizing minimal data representations and generalization. However, undecidability in finding these optimal representations and limits in data transmission impose constraints on \texttt{BCAI}’s scalability and efficiency. This chain reflects both the enabling and limiting aspects of \texttt{BCAI} development. Finally, we also find mini chains: 

\paragraph{$\bullet$ Limiting} Complexity Theorem $\mapsto$ Rice's Theorem and Chaitin’s Incompleteness Theorem $\mapsto$ G\"odel’s Incompleteness Theorem. In the first one, the Complexity Theory highlights that many real-world problems are computationally intractable, meaning that \texttt{BCAI} systems may struggle to efficiently solve critical tasks like optimization or decision-making. The Rice’s Theorem adds that even if solutions are found, verifying their correctness or safety is undecidable. Together, these theorems limit \texttt{BCAI}’s scalability and reliability in addressing complex problems and ensuring the quality of its outputs. In the second one, the G\"odel’s Incompleteness Theorem shows that \texttt{BCAI} systems, like any formal system, will encounter true statements they cannot prove, limiting their reasoning capabilities. The Chaitin’s Theorem further emphasizes that some truths require descriptions too complex for the system itself to process. These theorems collectively constrain \texttt{BCAI}’s ability to fully understand, optimize, or explain its own processes.
    
\paragraph{$\bullet$ Supporting} Algorithmic Information Theory $\mapsto$ Bayesian Inference and Hutter’s Universal AI $\mapsto$ Algorithmic Information Theory. In the first case, the Algorithmic Information Theory provides a framework for understanding data through its minimal representation, focusing on encoding efficiency and generalization. This aligns directly with Bayesian Inference, where models are updated to fit the data in the most probabilistically efficient way. The Algorithmic Information Theory supports Bayesian reasoning by enabling \texttt{BCAI} systems to prioritize simpler, more generalizable hypotheses, reducing overfitting and improving adaptability. However, the undecidability of finding truly minimal representations limits \texttt{BCAI}’s ability to fully optimize Bayesian models in practice. In the second case, the Hutter’s Universal AI relies on Algorithmic Information Theory to define an ideal decision-making agent. The Algorithmic Information theory underpins this model by focusing on the shortest possible description of environments, allowing the agent to generalize efficiently across tasks. While this highlights the theoretical potential of \texttt{BCAI}, the computational intractability of Solomonoff induction and the undecidability in the Algorithmic Information Theory create practical barriers, making the idealized agent infeasible for real-world implementation.

\begin{figure}[H]
    \centering
    \includegraphics[bb=0 0 600 800,width=0.6\linewidth]{images/BCAI.pdf}
    \caption[Relationships between computational theorems and their stance on \texttt{BCAI} feasibility]{Relationships between computational theorems and their stance on \texttt{BCAI} feasibility. The arrows represent how theorems interact conceptually. Colored nodes highlight enabling principles and emphasize intrinsic computational barriers, and white nodes present ambivalent Computational Intelligence theorems that can either aid or hinder \texttt{BCAI}.}
    \label{fig:BCAI_supp}
\end{figure}

Although some of these approaches may provide a theoretical path that could lead AI to \texttt{BCAI}, there are different kinds of issues (human and technical) that can influence its achievement, making the road to \texttt{TAI} a bumpy one. In the next part we analyze some of these \emph{potholes} that we are already facing today, as well as others that are looming on the horizon \citep{dobbe2024toward}. 
